The Dawn of Natural Language to SQL: Are We Fully Ready?

Translating users' natural language questions into SQL queries (i.e., NL2SQL) significantly lowers the barriers to accessing relational databases. The emergence of Large Language Models has introduced a novel paradigm in NL2SQL tasks, enhancing capabilities dramatically. However, this raises a critical question: Are we fully prepared to deploy NL2SQL models in production? To address the posed questions, we present a multi-angle NL2SQL evaluation framework, NL2SQL360, to facilitate the design and test of new NL2SQL methods for researchers. Through NL2SQL360, we conduct a detailed comparison of leading NL2SQL methods across a range of application scenarios, such as different data domains and SQL characteristics, offering valuable insights for selecting the most appropriate NL2SQL methods for specific needs. Moreover, we explore the NL2SQL design space, leveraging NL2SQL360 to automate the identification of an optimal NL2SQL solution tailored to user-specific needs. Specifically, NL2SQL360 identifies an effective NL2SQL method, SuperSQL, distinguished under the Spdier dataset using the execution accuracy metric. Remarkably, SuperSQL achieves competitive performance with execution accuracy of 87% and 62.66% on the Spider and BIRD test sets, respectively.

==> src/Q1.tex <==
\section{Who is the Winner: LLM-based or PLM-based Methods?}
\label{sec:q1}

\subsection{Setup}

\subsection{Accuracy \vs SQL Complexity}


\reminder{Table~\ref{tab:acc_sqlcomplexity}}

\begin{table}[h!]
	\centering
	\caption{Accuracy \vs SQL Complexity.}
	\label{tab:acc_sqlcomplexity}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|c|c|ccccc|}
			\hline
			\multirow{2}{*}{\textbf{Methods}} &
			\multirow{2}{*}{\textbf{Metrics}} &
			\multicolumn{5}{c|}{\textbf{Spider-Dev}} \\ \cline{3-7} 
			&
			&
			\multicolumn{1}{c|}{\textbf{Easy}} &
			\multicolumn{1}{c|}{\textbf{Medium}} &
			\multicolumn{1}{c|}{\textbf{Hard}} &
			\multicolumn{1}{c|}{\textbf{Extra}} &
			\textbf{All} \\ \hline \hline
			\multirow{2}{*}{C3-SQL} &
			EX &
			\multicolumn{1}{c|}{92.7} &
			\multicolumn{1}{c|}{85.2} &
			\multicolumn{1}{c|}{77.6} &
			\multicolumn{1}{c|}{62.0} &
			82.0 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{80.2} &
			\multicolumn{1}{c|}{43.5} &
			\multicolumn{1}{c|}{35.6} &
			\multicolumn{1}{c|}{18.1} &
			\multicolumn{1}{c|}{46.9} \\ \hline
			\multirow{2}{*}{DIN-SQL} &
			EX &
			\multicolumn{1}{c|}{92.3} &
			\multicolumn{1}{c|}{87.4} &
			\multicolumn{1}{c|}{76.4} &
			\multicolumn{1}{c|}{62.7} &
			82.8 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{82.7} &
			\multicolumn{1}{c|}{65.5} &
			\multicolumn{1}{c|}{42.0} &
			\multicolumn{1}{c|}{30.7} &
			\multicolumn{1}{c|}{60.1} \\ \hline
			\multirow{2}{*}{DAIL-SQL} &
			EX &
			\multicolumn{1}{c|}{91.5} &
			\multicolumn{1}{c|}{89.2} &
			\multicolumn{1}{c|}{77.0} &
			\multicolumn{1}{c|}{60.2} &
			83.1 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{89.5} &
			\multicolumn{1}{c|}{74.2} &
			\multicolumn{1}{c|}{55.5} &
			\multicolumn{1}{c|}{45.2} &
			\multicolumn{1}{c|}{70.0} \\ \hline
			\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DAIL-SQL\\ (with Self-Consistency)\end{tabular}} &
			EX &
			\multicolumn{1}{c|}{91.5} &
			\multicolumn{1}{c|}{90.1} &
			\multicolumn{1}{c|}{75.3} &
			\multicolumn{1}{c|}{62.7} &
			83.6 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{88.3} &
			\multicolumn{1}{c|}{73.5} &
			\multicolumn{1}{c|}{54.0} &
			\multicolumn{1}{c|}{41.6} &
			\multicolumn{1}{c|}{68.7} \\ \hline
			\multirow{2}{*}{RESDSQL   + NatSQL} &
			EX &
			\multicolumn{1}{c|}{94.4} &
			\multicolumn{1}{c|}{87.9} &
			\multicolumn{1}{c|}{77.0} &
			\multicolumn{1}{c|}{66.3} &
			84.1 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{93.1} &
			\multicolumn{1}{c|}{83.0} &
			\multicolumn{1}{c|}{70.1} &
			\multicolumn{1}{c|}{65.7} &
			\multicolumn{1}{c|}{80.5} \\ \hline
			\multirow{2}{*}{Graphix   + PICARD} &
			EX &
			\multicolumn{1}{c|}{92.3} &
			\multicolumn{1}{c|}{86.3} &
			\multicolumn{1}{c|}{73.6} &
			\multicolumn{1}{c|}{57.2} &
			80.9 \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{91.9} &
			\multicolumn{1}{c|}{82.3} &
			\multicolumn{1}{c|}{65.5} &
			\multicolumn{1}{c|}{53.0} &
			\multicolumn{1}{c|}{77.1} \\ \hline
			\multirow{2}{*}{\textbf{HyperSQL   (ours)}} &
			EX &
			\multicolumn{1}{c|}{\textbf{93.1}} &
			\multicolumn{1}{c|}{\textbf{90.1}} &
			\multicolumn{1}{c|}{\textbf{83.3}} &
			\multicolumn{1}{c|}{\textbf{66.3}} &
			\textbf{85.9} \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{91.9} &
			\multicolumn{1}{c|}{74.2} &
			\multicolumn{1}{c|}{59.2} &
			\multicolumn{1}{c|}{35.5} &
			\multicolumn{1}{c|}{69.7} \\ \hline
			\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{HyperSQL (ours)}\\ \textbf{(with Self-Consistency)}\end{tabular}} &
			EX &
			\multicolumn{1}{c|}{\textbf{94.4}} &
			\multicolumn{1}{c|}{\textbf{91.3}} &
			\multicolumn{1}{c|}{\textbf{83.3}} &
			\multicolumn{1}{c|}{\textbf{68.7}} &
			\textbf{87.0} \\ \cline{2-7} 
			&
			EM &
			\multicolumn{1}{c|}{90.3} &
			\multicolumn{1}{c|}{76.7} &
			\multicolumn{1}{c|}{61.5} &
			\multicolumn{1}{c|}{44.0} &
			\multicolumn{1}{c|}{72.1} \\ \hline
		\end{tabular}%
	}
\end{table}



\subsection{Accuracy \vs SQL Characteristics}

\reminder{Figure~\ref{fig:acc_sql_char}, Figure~\ref{fig:acc_sql_char2}}



\begin{figure*}[h!]
	%	\hspace*{-1.5em}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/expr/acc_sql/acc_sql_char.pdf}
	\vspace*{-2em}
	\caption{Execution Score \vs SQL Characteristics \red{Rank by stability?}.}
	\label{fig:acc_sql_char}
\end{figure*}

\begin{figure*}[h!]
	%	\hspace*{-1.5em}
	\centering
	\includegraphics[width=1.0\textwidth]{figures/expr/acc_sql/acc_sql_char_2.pdf}
	\vspace*{-2em}
	\caption{Execution Score \vs SQL Characteristics (Partition Spider Dev by Two Conditions).}
	\label{fig:acc_sql_char2}
\end{figure*}


\subsection{Main Findings}


\redfont{
	\be
	\item Currently, no LLM-based methods significantly surpass the PLM-based methods.
	\item No single \nlsql method consistently performs as the best across various types of SQL queries
	\item Pre-training can improve the capability of the \nlsql solution, especially when there are multiple JOIN conditions and Predicates.
	\item Although LLM-based Solutions can achieve the highest average score, PLM-based Methods can better handle different types of SQL and have a better understanding of the database Schema.
	\item Exploring the use of models such as GPT-4 through prompting engineering is not a long-term solution. If we really want to employ \nlsql method in production, then pre-training is very necessary.
	\item  In actual applications, accuracy cannot be the only factor in evaluating the quality of \nlsql. In addition, we also need to consider the stability and interpretability of the \nlsql solution.
	\item Interleaving the use of PLM and LLM in \nlsql represents a promising approach to achieve competitive results while balancing cost and efficiency.
	\ee
}

==> src/Q2.tex <==
\section{Is Accuracy Sufficient to Evaluate NL2SQL Solutions?}
\label{sec:q2}

\subsection{Setup}

\bluefont{Additionally, potential biases in existing NL2SQL benchmarks can lead to skewed comparisons, resulting in an incomplete or misleading portrayal of a method's true efficacy. Such biases might arise from over-representation of certain types of queries, lack of diversity in the databases used for testing, or benchmark datasets that do not adequately mirror the complexity and variability of real-world data. This can lead to the overestimation of certain methods that are tailored to the specifics of the benchmark, while underrepresenting the capabilities of methods that may be more adaptable or effective in a broader range of practical applications.}

\subsection{Question Understanding Ability}
\label{sub:questionUnderstanding}

\reminder{Accuracy of LLMs/PLM-based Methods by rephrasing NL query.}

\stitle{Exp-X: Rephrase Natural Language Query.}

\stitle{Exp-X: Ambiguous Natural Language Query.}

\subsection{Economy of LLMs-based Methods}

\begin{table*}[]
\centering
\caption{Accuracy vs. LLM Economy.}
\label{tab:llm-economy}
%\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Method}
&
\textbf{GPT Type}
& 
\begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{Input Tokens}\end{tabular} 
& 
\begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{Output Tokens}\end{tabular}
&
\begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{Total Tokens}\end{tabular}
&
\begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{Cost}\end{tabular}
&
\textbf{EX}
\\ \hline \hline
ChatGPT~\cite{liu2023comprehensive}              & gpt-3.5-turbo  & 158.33               & 39.60                  & 197.93               & 0.00024          & 70.1               \\ \hline
C3-SQL~\cite{dong2023c3}               & gpt-3.5-turbo  & 1061.73              & 4640.33               & 5702.07              & 0.01034          & 82.0               \\ \hline 
DIN-SQL~\cite{pourreza2023din}              & gpt-4          & 9181.00               & 389.80                 & 9570.80               & 0.29882          & 82.8               \\ \hline
DAIL-SQL~\cite{gao2023text}             & gpt-4          & 898.73               & 31.07                 & 929.80                & 0.02883          & 83.1               \\ \hline
\begin{tabular}[c]{@{}c@{}}DAIL-SQL~\cite{gao2023text}\\ (with Self-Consistency)\end{tabular}          & gpt-4          & 867.47               & 195.20                 & 1062.67              & 0.03774          & 83.6               \\ \hline
\textbf{HyperSQL (ours)}    & \textbf{gpt-4} & \textbf{687.20}       & \textbf{40.73}        & \textbf{727.93}      & \textbf{0.02306} & \textbf{85.9}      \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{HyperSQL (ours)}\\ \textbf{(with Self-Consistency)}\end{tabular} & \textbf{gpt-4} & \textbf{703.20}       & \textbf{238.60}        & \textbf{941.80}       & \textbf{0.03541} & \textbf{87.0}      \\ \hline
\end{tabular}
%}
\end{table*}

\reminder{Accuracy \vs \#-Tokens}

Table \ref{tab:llm-economy}


\subsection{Efficiency of PLM-based Methods}

\reminder{Accuracy \vs Latency}

\reminder{Accuracy \vs Model Size}

\subsection{Domain Adaption Ability}

\stitle{Findings.}
\bi
\item (1) LLMs exhibit superior generalization capabilities compared to fine-tuned models, particularly in downstream tasks involving out-of-distribution data. 

\item (2) LLMs are generally more effective than fine-tuned models in contexts with limited annotated data. However, when abundant annotated data is available, the choice between LLMs and fine-tuned models should be guided by the specific requirements of the task at hand.

\item (3) For optimal results, it is advisable to select models that have been pre-trained on datasets similar to the data encountered in downstream tasks.
\ei

\subsection{SQL Efficiency - Valid Efficiency Score}

Table \ref{tab:sql-ves}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\caption{The Valid Efficiency Score (VES) comparison in Spider.}
\label{tab:sql-ves}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|ccccc|}
\hline
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c|}{\textbf{Spider-Dev}}                                                                                  \\ \cline{2-6} 
 &
  \multicolumn{1}{c|}{\textbf{Easy}} &
  \multicolumn{1}{c|}{\textbf{Medium}} &
  \multicolumn{1}{c|}{\textbf{Hard}} &
  \multicolumn{1}{c|}{\textbf{Extra}} &
  \textbf{All} \\ \hline \hline
C3-SQL~\cite{dong2023c3}                            & \multicolumn{1}{c|}{93.10}  & \multicolumn{1}{c|}{75.29} & \multicolumn{1}{c|}{79.19} & \multicolumn{1}{c|}{59.82} & 77.74 \\ \hline
DIN-SQL\cite{pourreza2023din}                           & \multicolumn{1}{c|}{93.53} & \multicolumn{1}{c|}{79.94} & \multicolumn{1}{c|}{78.60}  & \multicolumn{1}{c|}{63.69} & 80.36 \\ \hline
DAIL-SQL\cite{gao2023text}                          & \multicolumn{1}{c|}{93.12} & \multicolumn{1}{c|}{79.61} & \multicolumn{1}{c|}{81.33} & \multicolumn{1}{c|}{60.31} & 80.04 \\ \hline
\begin{tabular}[c]{@{}c@{}}DAIL-SQL~\cite{gao2023text}\\ (with Self-Consistency)\end{tabular} &
  \multicolumn{1}{c|}{92.38} &
  \multicolumn{1}{c|}{81.11} &
  \multicolumn{1}{c|}{79.73} &
  \multicolumn{1}{c|}{62.73} &
  80.63 \\ \hline
RESDSQL + NatSQL~\cite{li2023resdsql}                  & \multicolumn{1}{c|}{94.69} & \multicolumn{1}{c|}{79.85} & \multicolumn{1}{c|}{77.06} & \multicolumn{1}{c|}{67.59} & 80.97 \\ \hline
Graphix + PICARD                  & \multicolumn{1}{c|}{91.93} & \multicolumn{1}{c|}{78.92} & \multicolumn{1}{c|}{72.50}  & \multicolumn{1}{c|}{57.97} & 77.59 \\ \hline
\textbf{HyperSQL (ours)} &
  \multicolumn{1}{c|}{\textbf{94.41}} &
  \multicolumn{1}{c|}{\textbf{81.25}} &
  \multicolumn{1}{c|}{\textbf{87.05}} &
  \multicolumn{1}{c|}{\textbf{64.49}} &
  \textbf{82.69} \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{HyperSQL (ours)}\\ \textbf{(with Self-Consistency)}\end{tabular} &
  \multicolumn{1}{c|}{\textbf{94.83}} &
  \multicolumn{1}{c|}{\textbf{81.29}} &
  \multicolumn{1}{c|}{\textbf{83.97}} &
  \multicolumn{1}{c|}{\textbf{65.36}} &
  \textbf{82.43} \\ \hline
\end{tabular}%
}
\end{table}

\subsection{Main Findings}




==> src/data.tex <==

\section{Data Construction}
\label{sec:data}




==> src/experiment.tex <==

\section{Additional Experiment}
\label{sec:experiment}



\subsection{Benchmark Dataset Exploration}

\add{Add a figure to show the distribution of Spider dataset.}

\add{Discuss the bias of current metrics according to data set distribution.}

Figure~\ref{fig:dataset_heatmap} and Figure~\ref{fig:dataset_dist}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.\textwidth]{figures/dataset_heatmap.pdf}
	\caption{SQL Characteristics in Spider Dataset.}
	\label{fig:dataset_heatmap}
\end{figure*}




\begin{figure}[t!]
	\centering
	\includegraphics[width=1.05\columnwidth]{figures/dataset_dist5.pdf}
	\caption{SQL Characteristics in Spider Dataset.}
	\label{fig:dataset_dist}
\end{figure}




\begin{figure}[t!]
	\centering
	\includegraphics[width=1\columnwidth]{figures/sqlhardness.pdf}
	\caption{SQL Hardness vs. in Spider Sources.}
	\label{fig:sql_hardness}
\end{figure}




\subsection{Database Schema Design}

Clear Schema \vs Ambiguous Schema




% \begin{lstlisting}[mathescape, float=t, caption=Ambiguous Schema]
	
% Question:
%  /*
% What is the maximum capacity and 
% the average of all stadiums ?
% */

% Predict SQL: 
% SELECT MAX(Capacity), AVG(Capacity) 
% FROM stadium

% Gold SQL:  
% select max(capacity), average from stadium

% Schema: 

% CREATE TABLE "stadium" (
% "Stadium_ID" int,
% "Location" text,
% "Name" text,
% "Capacity" int,
% "Highest" int,
% "Lowest" int,
% "Average" int,
% PRIMARY KEY ("Stadium_ID")
% );
% \end{lstlisting}
